Acoustic power absorption and enhancement generated by slow and fast MHD waves

We used long duration, high quality, unresolved (Sun-as-a star) observations collected by the ground based network BiSON and by the instruments GOLF and VIRGO on board the ESA/NASA SOHO satellite to search for solar-cycle-related changes in mode characteristics in velocity and continuum intensity for the frequency range between 2.5mHz < nu < 6.8mHz. Over the ascending phase of solar cycle 23 we found a suppression in the p-mode amplitudes both in the velocity and intensity data between 2.5mHz <nu< 4.5mHz with a maximum suppression for frequencies in the range between 2.5mHz <nu< 3.5mHz. The size of the amplitude suppression is 13+-2 per cent for the velocity and 9+-2 per cent for the intensity observations. Over the range 4.5mHz <nu< 5.5mHz the findings hint within the errors to a null change both in the velocity and intensity amplitudes. At still higher frequencies, in the so called High-frequency Interference Peaks (HIPs) between 5.8mHz <nu < 6.8mHz, we found an enhancement in the velocity amplitudes with the maximum 36+-7 per cent occurring for 6.3mHz <nu< 6.8mHz. However, in intensity observations we found a rather smaller enhancement of about 5+-2 per cent in the same interval. There is evidence that the frequency dependence of solar-cycle velocity amplitude changes is consistent with the theory behind the mode conversion of acoustic waves in a non-vertical magnetic field, but there are some problems with the intensity data, which may be due to the height in the solar atmosphere at which the VIRGO data are taken.

==> PaxHeader/13091mn.tex <==
18 gid=2048330233
17 uid=174949570
20 ctime=1271673205
20 atime=1271750624
38 LIBARCHIVE.creationtime=1271318825
24 SCHILY.dev=234881026
22 SCHILY.ino=2565528
18 SCHILY.nlink=1

